Bounded Verification with On-the-Fly Discrepancy Computation

Simulation-based verification algorithms can provide formal safety guarantees for nonlinear and hybrid systems. The previous algorithms rely on user provided model annotations called discrepancy function, which are crucial for computing reachtubes from simulations. In this paper, we eliminate this requirement by presenting an algorithm for computing piece-wise exponential discrepancy functions. The algorithm relies on computing local convergence or divergence rates of trajectories along a simulation using a coarse over-approximation of the reach set and bounding the maximal eigenvalue of the Jacobian over this over-approximation. The resulting discrepancy function preserves the soundness and the relative completeness of the verification algorithm. We also provide a coordinate transformation method to improve the local estimates for the convergence or divergence rates in practical examples. We extend the method to get the input-to-state discrepancy of nonlinear dynamical systems which can be used for compositional analysis. Our experiments show that the approach is effective in terms of running time for several benchmark problems, scales reasonably to larger dimensional systems, and compares favorably with respect to available tools for nonlinear models.

==> ContractionAnalysis.tex <==
\section{Contraction analysis of systems} \label{Contraction_analysis}
Consider the dynamic system
\begin{equation}\label{dynamic system 2}
\dot \vx = f(\vx,t)
\end{equation}
where $f: \mathbb{R}^n \times \mathbb{R}^{\geq 0} \rightarrow \mathbb{R}^n $

Consider two neighboring trajectories $\xi (\vx_{10},t), \xi(\vx_{20},t) \in \mathbb{R}^n \times \mathbb{R}^{\geq 0}$ starting  from $\vx_{10}(\xi(\vx_{10},t_1))$ and $\vx_{20} (\xi(\vx_{20},t_1))\in \mathbb{R}^n$.

Let $\delta \vx(t) = \xi (\vx_{10},t) - \xi(\vx_{20},t)$ and $\delta \vx_0 = \vx_{10}- \vx_{20}$, that is, $\delta \vx$  is the distance between two neighboring trajectories starting from two different initial points. From \cite{slotine98} we know
%The plant Equation\eqref{dynamic system 2}can be thought of as an $n$-dimensional fluid flow, where $\dot x$ is the $n$-dimensional "velocity" vector at the $n$-dimensional position $x$ and time $t$. We can get that
\begin{equation}\label{partial function}
\delta \dot \vx(t) =\frac{\partial f}{\partial \vx}(\vx,t)\delta \vx(t)
\end{equation}
%where $\delta x$ is a virtual displacement at fixed time, which is the distance between two neighboring trajectories starting from two different initial points.

Formally, $\delta \vx$ defines a linear tangent differential form, and $\delta \vx^{T}\delta \vx$ the associated quadratic tangent form.

From Proposition \ref{Lambda_max}, the rate of change in certain region $S,[t_1,t_2]$ should be:
\begin{equation}\label{quadratic form differential}
\begin{split}
\frac{d}{dt}(\delta \vx^{T}\delta \vx) & = \delta \dot \vx^{T}\delta \vx + \delta \vx^{T}\delta \dot \vx \\
&= \delta \vx^T \frac{\partial f^T}{\partial \vx}(\vx,t) \delta \vx + \delta \vx^T \frac{\partial f}{\partial \vx}(\vx,t) \delta \vx \\
&=\delta \vx^{T}(\frac{\partial f^T}{\partial \vx}(\vx,t) +\frac{\partial f}{\partial \vx}(\vx,t) )\delta \vx  \\
&=2\delta \vx J(\vx,t) \delta \vx \leq 2 \lambda_{max}(S,[t_1,t_2])\delta \vx^{T}\delta \vx
\end{split}
\end{equation}

where $\lambda_{max}(S,[t_1,t_2])$is the upper bound of the eigenvalues of the symmetric part of the Jacobian matrix, i.e. $\frac{1}{2}(\frac{\partial f^T}{\partial \vx}(\vx,t) +\frac{\partial f}{\partial \vx}(\vx,t)) $, from \eqref{quadratic form differential} we can get:
\begin{equation}\label{convergence rate}
\begin{split}
\frac{d(\delta \vx^T \delta \vx)}{\delta \vx^T \delta \vx} \leq 2\lambda_{max}(S,[t_1,t_2])dt \\
\end{split}
\end{equation}

Integrate each side from $t_1$ to $t \in [t_1,t_2]$:
\begin{equation}\label{convergent rate 2}
\begin{split}
&\ln (\delta \vx(t)^T \delta \vx(t))-\ln(\delta \vx(t_1)^T \delta \vx(t_1)) \leq 2\lambda_{max}(S,[t_1,t_2])(t-t_1) \\
\Rightarrow &\delta \vx(t)^T \delta \vx(t) \leq e^{2\lambda_{max}(S,[t_1,t_2])(t-t_1)}\delta \vx_0^T \delta \vx_0 \\
\Rightarrow & \|\delta \vx(t)\|^2 \leq e^{2\lambda_{max}(S,[t_1,t_2])(t-t_1)} \|\delta \vx_0\|^2 \\
\Rightarrow & \|\delta \vx(t)\| \leq \|\delta x_{0}\|e^{\lambda_{max}(S,[t_1,t_2])(t-t_1)}
\end{split}
\end{equation}
%A region of the state space is called a contraction region if the Jacobian matrix is uniformly negative definite in that region. By uniformly negative definite we mean that

When Jacobian is not uniformly negative definite, \eqref{convergent rate 2} can also show the divergence rate of two neighboring trajectories. This is what we want to use as the discrepancy function.

==> algorithm.tex <==
% !TEX root = main.tex
\section{Algorithms}
%\begin{figure}
%\begin{center}
%\begin{algorithmic}[1]
%\STATE {\bf Input:}  $\delta_0$, $\tup{f,\Theta,U}$, $\omega$, $T_{b}$
%\STATE $S \gets \Theta$; $\delta \gets \delta_0$; $\R \gets \emptyset$
%\WHILE{$S \neq \emptyset$}
%  \STATE $\X \gets \delta\mbox{-Partition}(S)$ \label{ln:1}
%  \FOR {$x_0 \in \X$}
%    \STATE $\epsilon \gets \sup\{\beta(y,x_0,t) \: |\:
%                  y \in B_\delta(x_0),\ 0 \leq t \leq T_{b}\}$ \label{ln:sup}
%    \STATE $\epsilon' \gets \sup\{\beta(y,x_0,t) |
%                  y \in B_{(\omega+\delta)}(x_0),\ 0 \leq t \leq T_{b}\}$ \label{ln:sup2}
%    \STATE $\psi \gets
%    \mbox{simulate}(x_0,T_{b},\epsilon,\tau)$ \label{ln:2}
%    \STATE $V(x_1,x_2),(\alpha_1,\alpha_2,\beta) \gets GetAnnotation(\psi,\tup{f,S},\mbox{step})$
%    \STATE $\T \gets B^V_\epsilon(\psi)$ \label{ln:3}
%    \IF {$\T \cap U = \emptyset$} \STATE $S \gets S \setminus B_\delta(x_0)$; $\R \gets \R \cup \T$ \label{ln:4}
%    \ELSIF {$\exists i.\ B^V_{\epsilon'}(R_i) \subseteq U$} \label{ln:condunsafe}
%       \RETURN (UNSAFE, $\R$, $max \{ 2\epsilon + \epsilon' \}$) \label{ln:5}
%    \ELSIF {$\exists i.\ R_i \subseteq U$ \AND $\ B^V_{\epsilon'}(R_i) \nsubseteq U$ }
%       \RETURN ($\omega$-TOO LARGE, $\R$, $max \{ 2\epsilon + \epsilon'\}$) \label{ln:5add}
%    \ENDIF
%  \ENDFOR
%  \STATE $\delta \gets \delta/2$; $\tau \gets \tau/2$
%\ENDWHILE
%\RETURN (SAFE, $\R$, $max \{ 2\epsilon + \epsilon'\}$) \label{ln:saferet}
%\end{algorithmic}
%\caption{Algorithm 1: Safety verification of dynamical systems.}
%\label{fig:verification algorithm}
%\end{center}
%\end{figure}
\begin{definition} \label{def:simulation}
Given a dynamical system $A$, an initial state $\theta$, a time bound $T$, and error bound $\epsilon >0$, and time step $\tau >0$, for $\xi =Traj(A,\theta)$, a $(\theta,T,\epsilon,\tau)$-simulation trace is a finite sequence $\phi=(R_0,t_0),(R_1,t_1),\dots,(R_l,t_l)$ where
\begin{enumerate}[(i)]
\item $t_0 = 0,t_l = T,$ and $\forall k \in \{1,2,\dots,l\}, t_i - t_{i-1} \leq \tau$
\item $\forall k \in \{1,2,\dots,l\}$ and $\forall t \in [t_{k-1},t_k]$, $\xi(t)\in R_{k}$
\item $\forall k \in \{0,1,2,\dots,l\}$,dia($R_{k}\leq \epsilon$)
\end{enumerate}
\end{definition}
In Algorithm \ref{alg:main}, the subroutine $\mathit{Simulate}(A,\theta,T,\epsilon,\tau)$(line \ref{al1:simulation}) computes a $(\theta,T,\epsilon,\tau)$-simulation as in Definition \ref{def:simulation}.


\begin{algorithm}[h!]
\caption{Verifying dynamic systems}
\label{alg:main}
\SetKwInOut{Input}{input}
%%%
\Input{$A,\unsafe,\epsilon_0,\delta_0,T$}
%%
$\delta \gets \delta_0; \epsilon\gets \epsilon_0; \R\gets \emptyset$\;
$\C   \gets \mathit{Partition}(\Theta_\A,\delta,\epsilon)$\;   \label{al1:partition}
\While{ $\C \neq \emptyset $
}{ 	
	\For{$(\theta,\delta,\epsilon)\in \X$}{
		%$(r_1,r_2,r'_1,r'_2) \gets \mbox{Bound}(M,\delta,\omega,T,\epsilon,\tau)$\;
		$\psi \gets \mathit{Simulate}(A, \theta, T, \epsilon,\tau)$\; \label{al1:simulation}
		%$M\gets \mathit{ISApprox}(\delta,\{V_i,\lalpha_i,\ualpha_i,\beta_i,\gamma_{ij}\})$\;  \label{ln:defM}
		%$\phi \gets \mathit{Simulate}(M, \theta_M, T, \epsilon,\tau)$\; \label{ln:getMtrace}
		%$\rho \gets \mathit{SupByTime}(\phi)$\; \label{ln:getrho}
		%$r_1 \gets  \sup\{(M_1)_i\} +\epsilon;$ $r_2\gets \sup\{ (M_2)_i\} +\epsilon$\;
                  %$\{V_i,\lalpha_i,\ualpha_i,\beta_i,\gamma_{ij}\} \gets GetAnnotation(\psi,\tup{f,S},\mbox{step})$\;
		%$S \gets B^{V}_{\rho}(\psi)$\; \label{ln:ball}
		S $\gets$ ALG2($\psi$,Jac,$f,\delta$)\;
		\uIf{$S \cap \unsafe =\emptyset$}{
			$\C\gets \C\backslash\{(\theta,\delta,\epsilon)\} ; \R \gets \R \cup S$ \; \label{al1:unsafe}
		}
		\uElseIf{$\exists k, R_k \subseteq \unsafe$}{
			\Return $(\mbox{UNSAFE},\R)$
		}
		\Else{
		$\C \gets \C \backslash \{(\theta,\delta,\epsilon)\}$\;	
		$ \C \gets \C \cup \mathit{Partition}(\Theta\cap B_\delta(\theta),(\frac{\delta_1}{2},\dots,\frac{\delta_N}{2}),\frac{\epsilon}{2})$\;
		}
		
	}
	

}
\Return $(\mbox{SAFE},\R)$\;
\end{algorithm}


For any state $\vx \in \mathbb{R}^n$ we define $B_{\delta}^{V}(\vx) \triangleq \{ \vy | V(\vx,\vy) \leq \delta \}$. For a subset $W \subseteq \mathbb{R}^{n}$, $B_{\delta}^{W} \triangleq \cup_{\vx \in W}B_{\delta}^{V}(\vx)$.


\begin{algorithm}[h!]
\caption{GetAnnotation function}
\SetKwInOut{Input}{input}
\Input {$\psi$,Jac,$f,\delta$}
E $\gets$ $\emptyset$ \;
%\STATE {Jac$(\vx,t) = \frac{\partial f(\vx,t)}{\vx}$}
\For {i = 1:length($\psi$)-1}
    %\STATE {du $\gets$ $t_{\textrm{i}}-t_{\textrm{i+1}}$}
   { {S $\gets$ $\{\vx | \forall t \in [t_\textrm{i},t_\textrm{i+1}], \exists \vy \in (R_i \cup R_{i+1}), \| \vx - \vy \| \leq e^{L_{f}(t-t_\textrm{i})} \delta \}$ }\;
    {s$_0$ $\gets$ center(S)}\;
    {J $\gets$ Jac(s$_0)$}\;
    {$\lambda$ $\gets$ max(eigenvalue(${\textrm{J}}$+${\textrm{J}}$$^T$)/2)}\;
    {error $\gets$ $\max \limits_{\forall \vx \in \textrm{S}}$ ((Jac($\vx,t$)+Jac$^T(\vx,t)$)-(${\textrm{J}}$+${\textrm{J}}$$^T$))}\;
    {$\lambda_{\textrm{max}}$ $\gets$ $\lambda$ + error/2}\;
   % \STATE {$\gamma[\textrm{i}] $ $\gets$ $\lambda_{\mbox{max}}$}
    {U$_\textrm{i}$ $\gets$ $\{\vx | \forall t \in [t_\textrm{i},t_\textrm{i+1}],\exists \vy \in (R_i \cup R_{i+1}), \| \vx - \vy \| \leq e^{\lambda_{\textrm{max}}(t-t_\textrm{i}) } \delta \}$ }\;
    {E $\gets$ E $\cup$ $\tup{\textrm{U}_\textrm{i},[t_\textrm{i},t_\textrm{i+1}]}$ }\;
    {$\delta$ $\gets$ $e^{\lambda_{\textrm{max}}(t_\textrm{i+1}-t_\textrm{i}) } \delta $}\;
}
\Return $\mbox{E}$ \;

\end{algorithm}




%\begin{figure}
%\begin{center}
%\begin{algorithmic}[1]
%\STATE {\bf Input:} $\psi$,$\tup{f,\Theta}$,step
%\STATE {Jac$(\vx,t) = \frac{\partial f(\vx,t)}{\vx}$}
%\FOR {cnt1 = 1:step:k}
%    \STATE {tb $\gets$min(cnt1+step-1,k)}
%    \STATE {Ave $\gets$ mean(Jac(center($R_{cnt1}$),$t_{cnt1}$),$\cdots$,Jac(center($R_{tb}$),$t_{tb}$))}
%    \STATE {M $\gets$ Similar transform(Ave), where J = MAveM$^{-1}$ and J is the Jordan form}
%    \STATE {$K[cnt1] $ $\gets$ cond(M)}
%    \STATE {$\Theta$ $\gets$ cond(M)}$\Theta$
%    \FOR {cnt2 = cnt1:tb}
%        \STATE {S $\gets$ Lip($\Theta,R_{cnt2},R_{cnt2+1},t_{cnt2},t_{cnt2+1}$) }
%        \STATE {J $\gets$ Jac$(\mbox{center}(R_{cnt2}),t_{cnt2})$}
%        \STATE {$\tilde{\textrm{J}}$ $\gets$ MJM$^{-1}$}
%        \STATE {$\lambda$ $\gets$ max(eigenvalue($\tilde{\textrm{J}}$+$\tilde{\textrm{J}}$$^T$)/2)}
%        \STATE {$\hat{\textrm{J}}$(S) $\gets$ $\forall \vx,t \in s:\mbox{Jac}(\vx,t)$}
%        \STATE {$\hat{\textrm{J}}$(S) $\gets$ M$\hat{\textrm{J}}$(S)M$^{-1}$}
%        \STATE {E(S) $\gets$  ($\hat{\textrm{J}}$(S)+$\hat{\textrm{J}}$$^T$(S))/2-($\tilde{\textrm{J}}$+$\tilde{\textrm{J}}$$^T$)/2}
%        \STATE {$\lambda_{\mbox{max}}$ $\gets$ $\lambda$ + max(E(S))}
%        \STATE {$\gamma[cnt2] $ $\gets$ $\lambda_{\mbox{max}}$}
%        \STATE {$\Theta$ $\gets$ $\Theta$ $\times$ $exp(\lambda_{\mbox{max}}(t_{cnt2+1}-t_{cnt2}))$}
%    \ENDFOR
%\ENDFOR
%\STATE {\bf Output:} $K$,$\gamma$
%
%\end{algorithmic}
%\caption{GetAnnotation function}
%\end{center}
%\end{figure}

\begin{lemma}
$\textrm{Reach}(B_{\delta}(x_0),[t_\textrm{i},t_\textrm{i+1}]) \subseteq $ S$_i (R_\textrm{i},R_\textrm{i+1},[t_\textrm{i},t_\textrm{i+1}])$
\end{lemma}

\begin{lemma}
$\textrm{Reach}(B_{\delta}(x_0),[t_\textrm{i},t_\textrm{i+1}]) \subseteq $ U$_\textrm{i}$
\end{lemma}


\begin{proposition}
Function "GetAnnotation" is correct. That is, it returns correct annotation for the discrepancy
\end{proposition}

\begin{proof}

\end{proof}

\begin{theorem}
\label{soundness}
Algorithm \ref{fig:verification algorithm} is sound. That is, if it returns "SAFE" then all the executions from $\Theta$ are safe, and when it returns "UNSAFE" there exists at least one execution from the initial set, that is safe
\end{theorem}

\begin{theorem}
\label{completness}
Algorithm~1 is a complete procedure for robust safety verification of dynamical systems.
That is, if all the executions from $\Theta$ are robustly safe, then the
it  will terminate and return ``SAFE''.
If any of the executions from $\Theta$ is unsafe, then it will terminate and return ``UNSAFE''.
\end{theorem}





==> prelude1.tex <==
\RequirePackage{amssymb}
\RequirePackage{tikz}
\let\oldemptyset\emptyset
\let\emptyset\varnothing
\let\mapsto\rightarrow
\let\cal\mathcal
\newcommand{\cross}{\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.15ex] \draw (0,0) -- (1,1) (0,1) -- (1,0);}}

%\newcommand{\mitras}[1]{\textcolor{blue}{#1}}
\newcommand{\mitras}[1]{{#1}}
% for nomencl to produce page links
%\renewcommand*{\pagedeclaration}[1]{\unskip, \hyperpage{#1}}
%\renewcommand{\nomname}{List of Symbols and Functions}

\newcommand{\authcomment}[1]{\textbf{[[#1]]}}
\newcommand{\sayan}[1]{\textcolor{blue}{\textbf{[SM: [#1]]}}}
\newcommand{\zhenqi}[1]{\textcolor{red}{#1}}
%\newcommand{\chuchu}[1]{\textcolor{red}{#1}}
%\newcommand{\sayan}[1]{}
\newcommand{\chuchu}[1]{}
%\newcommand{\taylor}[1]{\textcolor{red}{\textbf{[TJ: [#1]]}}}
\newcommand{\taylor}[1]{}
\newcommand{\jeremy}[1]{\textcolor{red}{\textbf{[JG: [#1]]}}}
%\newcommand{\jeremy}[1]{}


%FIXED SETS

%\newcommand{\Time}{{\sf T}}                     %time domain
\newcommand{\nnt}{{\sf T}^{\geq 0}}             %nonnegative time points
\newcommand{\post}{{\sf T}^{>0}}                %positive time points
\newcommand{\Variables}{{\sf V}}                %variables

\newcommand{\num}[1]{\relax\ifmmode \mathbb #1\else $\mathbb #1$\fi}
\newcommand{\nnnum}[1]{\relax\ifmmode
  {\mathbb #1}_{\geq 0} \else ${\mathbb #1}_{\geq 0}$
  \fi}
\newcommand{\npnum}[1]{\relax\ifmmode
  {\mathbb #1}_{\leq 0} \else ${\mathbb #1}_{\leq 0}$
  \fi}
\newcommand{\pnum}[1]{\relax\ifmmode
  {\mathbb #1}_{> 0} \else ${\mathbb #1}_{> 0}$
  \fi}
\newcommand{\nnum}[1]{\relax\ifmmode
  {\mathbb #1}_{< 0} \else ${\mathbb #1}_{< 0}$
  \fi}
\newcommand{\plnum}[1]{\relax\ifmmode
  {\mathbb #1}_{+} \else ${\mathbb #1}_{+}$
  \fi}
\newcommand{\nenum}[1]{\relax\ifmmode
  {\mathbb #1}_{-} \else ${\mathbb #1}_{-}$
  \fi}

\newcommand{\reals}{{\num R}}                    %reals
\newcommand{\booleans}{{\num B}}                    %reals
\newcommand{\nnreals}{{\nnnum R}}                    %nonnegative reals
\newcommand{\realsinfty}{{\num R} \cup \{\infty, -\infty\}}                    %nonnegative reals
\newcommand{\plreals}{{\plnum R}}                    %positive reals
\newcommand{\naturals}{{\num N}}                      %natural numbers
\newcommand{\integers}{{\num Z}}                      %integers
\newcommand{\rationals}{{\num Q}}                      %rationals
\newcommand{\nnrationals}{{\nnnum Q}}                   % nonnegative rationals
\newcommand{\Time}{{\num T}}

% EXECUTIONS TRACES and FRAGS
\newcommand{\extb}[1]{\relax\ifmmode {\sf ExtBeh}_{#1} \else ${\sf ExtBeh}_{#1}$\fi}
\newcommand{\tdists}[1]{\relax\ifmmode {\sf Tdists}_{#1} \else ${\sf Tdists}_{#1}$\fi}

\newcommand{\exec}[1]{\relax\ifmmode {\sf Execs}_{#1} \else ${\sf Exec}_{#1}$\fi}
\newcommand{\execf}[1]{\relax\ifmmode {\sf Execs}^*_{#1} \else ${\sf Exec}^*_{#1}$\fi}
\newcommand{\execi}[1]{\relax\ifmmode {\sf Execs}^\omega_{#1} \else ${\sf Exec}^\omega_{#1}$\fi}

\newcommand{\ctrace}[1]{\relax\ifmmode {\sf Ctraces}_{#1} \else ${\sf Ctraces}_{#1}$\fi}

\newcommand{\trace}[1]{\relax\ifmmode {\sf Traces}_{#1} \else ${\sf Traces}_{#1}$\fi}
\newcommand{\tracef}[1]{\relax\ifmmode {\sf Traces}^*_{#1} \else ${\sf Traces}^*_{#1}$\fi}
\newcommand{\tracei}[1]{\relax\ifmmode {\sf Traces}^\omega_{#1} \else ${\sf Traces}^\omega_{#1}$\fi}

\newcommand{\frag}[1]{\relax\ifmmode {\sf Frags}_{#1} \else ${\sf Frags}_{#1}$\fi}
\newcommand{\fragf}[1]{\relax\ifmmode {\sf Frags}^*_{#1} \else ${\sf Frags}^*_{#1}$\fi}
\newcommand{\fragi}[1]{\relax\ifmmode {\sf Frags}^\omega_{#1} \else ${\sf Frags}^\omega_{#1}$\fi}

\newcommand{\reach}[1]{\relax\ifmmode {\sf Reach}_{#1} \else ${\sf Reach}_{#1}$\fi}
\newcommand{\Reach}[1]{\relax\ifmmode {\sf Reach}_{#1} \else ${\sf Reach}_{#1}$\fi}

\newcommand{\execs}{{\exec{}}}
\newcommand{\traces}{{\trace{}}}
\newcommand{\fragss}{{\frag{}}}

\newcommand{\fexecs}{{\execf{}}}
\newcommand{\ftraces}{{\tracef{}}}
\newcommand{\ffragss}{{\fragf{}}}

\newcommand{\iexecs}{{\execi{}}}
\newcommand{\itraces}{{\tracei{}}}
\newcommand{\ifragss}{{\fragi{}}}

\newcommand{\val}[1]{\relax\ifmmode {\mbox{\it Val}}(#1) \else ${{\it Val}}({#1})$\fi}
\newcommand{\traj}[1]{\relax\ifmmode {\mathit Traj}(#1) \else ${\mathit Traj}({#1})$\fi}


%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newcounter{dcounter}
%\newtheorem{definition}[dcounter]{Definition}
%\newcounter{rcounter}
%\newtheorem{remark}[rcounter]{Remark}
%\newenvironment{noqed}{\pf}{}
%%\newcommand{\pf}{\par\noindent{\bf Proof:}~}
%
%\newtheorem{remark}{Remark}
%
%%\renewcommand{\thesubsection}{\arabic{subsection}}
% \newtheorem{theorem}{Theorem}
% %[subsection]
%%\newtheorem{lemma}[theorem]{Lemma}
% %\newtheorem{claim}[theorem]{Claim}
%%\theoremstyle{definition}
%\newcounter{dcounter}
%\newtheorem{definition}[dcounter]{Definition}
\renewcommand{\qed}{\hfill{\rule{2mm}{2mm}}\medskip}
%% \newenvironment{proof}{\pf}{\qed}
%\newtheorem{proposition}[theorem]{Proposition}
%%\newtheorem{invariant}[theorem]{Invariant}
% %\newtheorem{remark}[theorem]{Remark}
%%\theoremstyle{assumption}
\newcounter{asscounter}
\newtheorem{assumption}[asscounter]{Assumption}
%
%%\newcounter{invariant}



 %{\refstepcounter{theorem} \vspace{2ex}\par\noindent
 %\textbf{Example}~\textbf{\thetheorem~}}{\qed}

%\theoremstyle{remark}
 %\newcounter{ecounter}
 %\newtheorem{example}[ecounter]{Example}
% {\refstepcounter{theorem} \vspace{2ex}\par\noindent
% \textbf{Example}~\textbf{\theexampletheorem~}}{\qed}



% \examplenonum#1#2{
%	\vspace{.15in}
%	\noindent
%	{\bf Example #1}{\em ~(continued)}{\bf .}
%	{#2}{\qed}
%	}
%
% \renewcommand{\theequation}{\thesection.\arabic{equation}}
% \renewcommand{\thefigure}{\thesection.\arabic{figure}}
% \renewcommand{\thetable}{\thesection.\arabic{table}}
% \newcommand{\Section}[1]{\section{#1}%
%    \setcounter{equation}{0}\setcounter{figure}{0}\setcounter{table}{0}%
%    \setcounter{example}{0}}
%
% \newenvironment{anotation}[1][Nancy]{\begin{quote}\small[[[#1]]]}{\normalsize\end{quote}}
% \newcommand{\ba}{\begin{anotation}}
% \newcommand{\ea}{\end{anotation}}
%
% \newcommand{\bcb}{\chgbarbegin}
% \newcommand{\ecb}{\chgbarend}
% \chgbarwidth 1pt
%
% \newcommand{\dec}{\ensuremath{{:}}}
% \newcommand{\eqdef}{\mathbin{::=}}
% \newcommand{\I}{{\ensuremath{\cap}}}



% OPERATIONS ON SETS, RELATIONS AND FUNCTIONS
\newcommand{\pow}[1]{{\bf P}(#1)} % powerset
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\range}[1]{\ms{range{(#1)}}}
\newcommand{\domain}[1]{{\it dom}(#1)}
\newcommand{\type}[1]{\ms{type{(#1)}}}
\newcommand{\dtype}[1]{\ms{dtype{(#1)}}} % dynamic type
\newcommand{\restr}{\mathrel{\lceil}}
\newcommand{\proj}{\matrel{\lceil}}
\newcommand{\restrrange}{\mathrel{\downarrow}}
\newcommand{\point}[1]{\wp(#1)}     		%point trajectory



% HYBRID AUTOMATA
\def\A{{\cal A}} % HA
\def\B{{\cal B}} % HA
\def\C{{\cal C}} % HA
\def\D{{\cal D}} % set of discrete steps
\def\E{{\cal E}} % HA
\def\F{{\cal F}} % HA
\def\G{{\cal G}} % pieces of SHIOA
\def\H{{\cal H}} % HA
\def\I{{\cal I}} % environment sequence
\def\K{{\cal K}} % environment sequence
\def\L{{\cal L}} % lane
\def\M{{\cal M}} % Mode switching transitions
\def\N{{\cal N}}
\def\O{{\cal O}} % outcome function
\def\P{{\cal P}} % set of modes
\def\Q{{\cal Q}} % set of modes
\def\R{{\cal R}} % relation
\def\S{{\cal S}} % set of trajectories
\def\T{{\cal T}} % set of trajectories
\def\V{{\cal V}} % Lyapunov function
\def\U{{\cal U}} % set of trajectories
\def\X{{\cal X}} % Lyapunov function
\def\Y{{\cal Y}} % set of trajectories
\def\Z{{\cal Z}}

% hybrid automaton definitinos for ICCPS 2012
\def\Aq{\A_1}
\def\AL{\A_2}
\def\Ar{\A_3}
\def\Aall{\B}

% more special characters

\newcommand{\col}[1]{\relax\ifmmode \mathscr #1\else $\mathscr #1$\fi}

\def\statemodels{\col{S}}


% Names of actions, automata etc
\definecolor{HIOAcolor}{rgb}{0.776,0.22,0.07}
\newcommand{\HIOA}{\textcolor{HIOAcolor}{\tt HIOA\hspace{3pt}}}
\newcommand{\PVS}{\textcolor{HIOAcolor}{\tt PVS\hspace{3pt}}}
\newcommand{\PVSnogap}{\textcolor{HIOAcolor}{\tt PVS\hspace{1pt}}}
\newcommand{\HIOAbiggap}{\textcolor{HIOAcolor}{\tt HIOA\hspace{6pt}}}
\newcommand{\HIOAnogap}{\textcolor{HIOAcolor}{\tt HIOA}}
\newcommand{\anyrelation}{\lessgtr}

% Transformation for ADT
\newcommand{\SC}[2]{\relax\ifmmode {\tt Scount}(#1,#2) \else ${\tt Scount}(#1,#2)$\fi}
\newcommand{\SCM}[2]{\relax\ifmmode {\tt Smin}(#1,#2) \else ${\tt Smin}(#1,#2)$\fi}
\newcommand{\Aut}[1]{\relax\ifmmode {\tt Aut}(#1) \else ${\tt Aut}(#1)$\fi}

\newcommand{\auto}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\act}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\smodel}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\pvstheory}[1]{{\operatorname{\mathit{#1}}}}
%\newcommand{\auto}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}
%\newcommand{\act}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}


%\newcommand{\Automaton}{{\bf automaton}}
%\newcommand{\Asserts}{{\bf asserts}}
%\newcommand{\Assumes}{{\bf assumes}}
%\newcommand{\Backward}{{\bf backward}}
%\newcommand{\By}{{\bf by}}
%\newcommand{\Case}{{\bf case}}
%\newcommand{\Choose}{{\bf  choose}}
%\newcommand{\Components}{{\bf components}}
%\newcommand{\Const}{{\bf const}}
%\newcommand{\Converts}{{\bf converts}}
%\newcommand{\Do}{{\bf do}}
%\newcommand{\Eff}{{\bf eff}}
%\newcommand{\Else}{{\bf else}}
%\newcommand{\Elseif}{{\bf elseif}}
%\newcommand{\Enumeration}{{\bf enumeration}}
%\newcommand{\Ensuring}{{\bf ensuring}}
%\newcommand{\Exempting}{{\bf exempting}}
%\newcommand{\Fi}{{\bf fi}}
%\newcommand{\For}{{\bf for}}
%\newcommand{\Forward}{{\bf forward}}
%\newcommand{\Freely}{{\bf freely}}
%\newcommand{\From}{{\bf from}}
%\newcommand{\Generated}{{\bf generated}}
%\newcommand{\Local}{{\bf local}}
%\newcommand{\Hidden}{{\bf hidden}}
%\newcommand{\If}{{\bf if}}
%\newcommand{\In}{{\bf in}}
%\newcommand{\Implies}{{\bf implies}}
%\newcommand{\Includes}{{\bf includes}}
%\newcommand{\Introduces}{{\bf introduces}}
%\newcommand{\Input}{{\bf input}}
%\newcommand{\Kind}{{\bf kind}}
%\newcommand{\Initially}{{\bf initially}}
%\newcommand{\Internal}{{\bf internal}}
%\newcommand{\Invariant}{{\bf invariant}}
%\newcommand{\Od}{{\bf od}}
%\newcommand{\Of}{{\bf of}}
%\newcommand{\Output}{{\bf output}}
%\newcommand{\Partitioned}{{\bf partitioned}}
%\newcommand{\Pre}{{\bf pre}}
%\newcommand{\Signature}{{\bf signature}}
%\newcommand{\Simulation}{{\bf simulation}}
%\newcommand{\Sort}{{\bf sort}}
%\newcommand{\States}{{\bf states}}
%\newcommand{\Tasks}{{\bf tasks}}
%\newcommand{\Then}{{\bf then}}
%\newcommand{\To}{{\bf to}}
%\newcommand{\Trait}{{\bf trait}}
%\newcommand{\Traits}{{\bf traits}}
%\newcommand{\Transitions}{{\bf transitions}}
%\newcommand{\Tuple}{{\bf tuple}}
%\newcommand{\Type}{{\bf type}}
%\newcommand{\Union}{{\bf union}}
%\newcommand{\Uses}{{\bf uses}}
%\newcommand{\Where}{{\bf where}}
%\newcommand{\While}{{\bf while}}
%\newcommand{\With}{{\bf with}}


% Spacing
\newcommand{\FFF}{\vspace{0.1in}}
\newcommand{\BBB}{\hspace{-0.1in}}


% systematic labels
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter~\ref{ch:#1}}
\newcommand{\chreftwo}[2]{Chapters~\ref{ch:#1}~and~\ref{ch:#2}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\secreftwo}[2]{Sections~\ref{sec:#1}~and~\ref{sec:#2}}
\newcommand{\sslabel}[1]{\label{ss:#1}}
\newcommand{\ssref}[1]{Subsection~\ref{ss:#1}}
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\figreftwo}[2]{Figs.~\ref{fig:#1}~and~\ref{fig:#2}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\lnlabel}[1]{\label{line:#1}}
\newcommand{\lnsref}[2]{Lines~\ref{line:#1}--\ref{line:#2}\xspace}
\newcommand{\lnref}[1]{Line~\ref{line:#1}\xspace}
\newcommand{\lnreftwo}[2]{Lines~\ref{line:#1}~and~\ref{line:#2}\xspace}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}\xspace}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}\xspace}
\newcommand{\lemreftwo}[2]{Lemmata~\ref{lem:#1} and~\ref{lem:#2}\xspace}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}\xspace}
\newcommand{\corlabel}[1]{\label{cor:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}\xspace}
\newcommand{\invlabel}[1]{\label{inv:#1}}
\newcommand{\assref}[1]{Assumption~\ref{assump:#1}\xspace}
\newcommand{\assreftwo}[2]{Assumptions~\ref{assump:#1}~and~\ref{assump:#2}\xspace}
\newcommand{\asslabel}[1]{\label{assump:#1}}
%\renewcommand{\eqref}[1]{(\ref{eq:#1})\xspace}
\newcommand{\eqlabel}[1]{\label{eq:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}\xspace}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}\xspace}
\newcommand{\proplabel}[1]{\label{prop:#1}}
\newcommand{\exref}[1]{Example~\ref{ex:#1}\xspace}
\newcommand{\exlabel}[1]{\label{ex:#1}}
\newcommand{\ppageref}[1]{page~\pageref{#1}}
\newcommand{\conjref}[1]{Conjecture~\ref{conj:#1}\xspace}
\newcommand{\conjlabel}[1]{\label{conj:#1}}


% defs FROM ptioa PAPER


\newcommand{\remove}[1]{}
\newcommand{\salg}[1]{\relax\ifmmode {\mathcal F}_{#1}\else ${\mathcal F}_{#1}$\fi}
\newcommand{\msp}[1]{\relax\ifmmode (#1, \salg{#1}) \else $(#1, \salg{#1})$\fi}
\newcommand{\msprod}[2]{\relax\ifmmode ( #1 \times #2, \salg{#1} \otimes \salg{#2}) \else $(#1 \times #2, \salg{#1} \otimes \salg{#2})$\fi}
\newcommand{\dist}[1]{\relax\ifmmode {\mathcal P}\msp{#1}
  \else ${\mathcal P}\msp{#1}$\fi}
\newcommand{\subdist}[1]{\relax\ifmmode {\mathcal S}{\mathcal P}\msp{#1}
  \else ${\mathcal S}{\mathcal P}\msp{#1}$\fi}
\newcommand{\disc}[1]{\relax\ifmmode {\sf Disc}(#1)
  \else ${\sf Disc}(#1)$\fi}

\newcommand{\Trajeq}{\relax\ifmmode {\mathcal R}_\T \else ${\mathcal R}_\T$\fi}
\newcommand{\Acteq}{\relax\ifmmode {\mathcal R}_A \else ${\mathcal R}_A$\fi}
\newcommand{\noop}{\relax\ifmmode \lambda \else $\lambda$\fi}
\newcommand{\close}[1]{\relax\ifmmode \overline{#1} \else $\overline{#1}$\fi}

\newcommand{\corrtasks}{\mathop{\mathsf {c}}}
\newcommand{\full}{\mathop{\mathsf {full}}}
\newcommand{\fstate}{\mathop{\mathsf {fstate}}}
\newcommand{\lstate}{\mathop{\mathsf {lstate}}}
\newcommand{\ltime}{\mathop{\mathsf {ltime}}}
\newcommand{\dur}{\mathop{\mathsf {dur}}}
\newcommand{\tdist}{\mathop{\mathsf {tdist}}}
\newcommand{\extbeh}{\mathop{\mathsf {extbeh}}}
%\newcommand{\apply}{\mathop{\mathsf {apply}}}
\newcommand{\apply}[2]{\mathop{\mathsf {apply}({#1},{#2})}}
%\newcommand{\applytwo}{\mathop{\mathsf {apply2}}}
\newcommand{\support}{\mathop{\mathsf {supp}}}
\newcommand{\relation}{\mathrel{R}}
\newcommand{\cone}{C}
%\newcommand{\tracef}{\mathord{\mathsf {trace}}}
\newcommand{\flatten}{\mathord{\mathsf {flatten}}}
\newcommand{\discrete}{\mathord{\mathsf {Disc}}}
\newcommand{\lift}[1]{\mathrel{{\mathcal L}(#1)}}
\newcommand{\expansion}[1]{\mathrel{{\mathcal E}(#1)}}
%End of commands added by Roberto on May, 12

%>> Ling, December 2005

\newcommand{\subdisc}{\operatorname{\mathsf {SubDisc}}}
\newcommand{\tran}{\operatorname{\mathsf {tran}}}
%\newcommand{\act}{\operatorname{\mathsf {act}}}

\renewcommand{\execs}{{\operatorname{\mathsf {Execs}}}}
\newcommand{\frags}{{\operatorname{\mathsf {Frags}}}}

\newcommand{\tracefnc}{{\operatorname{\mathsf {trace}}}}

\newcommand{\finite}{{\operatorname{\mathsf {finite}}}}
\newcommand{\hide}{{\operatorname{\mathsf {hide}}}}

\newcommand{\early}{{\operatorname{\mathsf {Early}}}}
\newcommand{\late}{{\operatorname{\mathsf {Late}}}}
\newcommand{\toss}{{\operatorname{\mathsf {Toss}}}}

\newcommand{\define}{:=}

\newcommand{\pc}{{\operatorname{\mathsf {counter}}}}
\newcommand{\chosen}{{\operatorname{\mathsf {chosen}}}}

\newcommand{\rand}{{\operatorname{\mathsf {random}}}}
\newcommand{\unif}{{\operatorname{\mathsf {unif}}}}

\newcommand{\ie}{i.e.,\xspace}
\newcommand{\Ie}{I.e.,\xspace}

\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}

% IOA related stuff




\newcommand{\mybox}[3]{
  \framebox[#1][l]
  {
    \parbox{#2}
    {
      #3
    }
  }
}

\newcommand{\two}[4]{
  \parbox{.95\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{#3}%
    \parbox[t]{#2\columnwidth}{#4}%
  }}

\newcommand{\twosep}[4]{
  \parbox{\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{#3}%
   	\vrule width 0.2pt
    \parbox[t]{#2\columnwidth}{#4}%
  }}

\newcommand{\eqntwo}[4]{
  \parbox{\columnwidth}{\vspace{1pt} \vfill
    \parbox[t]{#1\columnwidth}{$ #3 $}
    \parbox[t]{#2\columnwidth}{$ #4 $}
  }}

\newcommand{\three}[6]{\vspace{1pt} \vfill
        \parbox{\columnwidth}{%
        \parbox[t]{#1\columnwidth}{#4}%
        \parbox[t]{#2\columnwidth}{#5}%
        \parbox[t]{#3\columnwidth}{#6}%
      }}

\newcommand{\tup}[1]
           {
             \relax\ifmmode
             \langle #1 \rangle
             \else $\langle$ #1 $\rangle$ \fi
           }

\newcommand{\lit}[1]{ \relax\ifmmode
                \mathord{\mathcode`\-="702D\sf #1\mathcode`\-="2200}
                \else {\it #1} \fi }


\newcommand{\figuresize}{\scriptsize}

\newcommand{\equationsize}{\footnotesize}

%\newcommand{\act}[1]{%
%  \relax\ifmmode
%                \mathord{\mathcode`\-="702D\sf #1\mathcode`\-="2200}%
%                \else
%                {\sf #1\/}%
%                \fi }


\lstdefinelanguage{ioa}{
  basicstyle=\figuresize,
  keywordstyle=\bf \figuresize,
  identifierstyle=\it \figuresize,
  emphstyle=\tt \figuresize,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  escapeinside={(*@}{@*)},
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={automaton,and, assumed,
  	 choose,const,continue, components,
  	 derived, discrete, do,
  	 eff, external,else, elseif, evolve, end,
  	 fi,for, each, foreach, forward, from,
  	 hidden,
  	 in,input,internal,if,invariant, initially, imports,
     let,
     or, output, operators, od, of,
     pre, private,
     return,
     satisfies, shared, signature, simulation, stop, such,
     trajectories,trajdef, transitions, that,then, type, types, to, tasks,
     variables, vocabulary,
     when,where, with,while},
  emph={Set, set, seq, tuple, map, array, enumeration},
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\nE}{{$\nexists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3
      }

\lstdefinelanguage{ioaNums}[]{ioa}
{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\lstdefinelanguage{ioaNumsRight}[]{ioa}
{
  numbers=right,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\newcommand{\ioa}{\lstinline[language=IOA]}

\lstnewenvironment{IOA}%
  {\lstset{language=IOA}}
  {}

\lstnewenvironment{IOANums}%
  {
  \if@firstcolumn
    \lstset{language=IOA, numbers=left, firstnumber=auto}
  \else
    \lstset{language=IOA, numbers=right, firstnumber=auto}
  \fi
  }
  {}

\lstnewenvironment{IOANumsRight}%
  {
    \lstset{language=IOA, numbers=right, firstnumber=auto}
  }
  {}

%\lstnewenvironment{IOA}%
%  {\lstset{language=ioaLang}
%   \csname lst@SetFirstLabel\endcsname}
%  {\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}

\newcommand{\figioa}[5]{
  \begin{figure}[#1]
      \hrule \F
      {\figuresize \bf #2}
      \lstinputlisting[language=ioaLang]{#5}
      \F \hrule \F
      \caption{#3}
      \label{fig: #4}
  \end{figure}
}

\newcommand{\linefigioa}[9]{

}

\newcommand{\twofigioa}[8]{
  \begin{figure}[#1]
    \hrule \F
    {\figuresize \bf #2} \\
    \two{#5}{#6}
    {
      \lstinputlisting[language=ioaLang]{#7}
    }
    {
      \lstinputlisting[language=ioaLang]{#8}
    }
    \F \hrule \F
    \caption{#3}
    \label{fig: #4}
  \end{figure}
}



\lstdefinelanguage{ioaLang}{%
  basicstyle=\ttfamily\small,
  keywordstyle=\rmfamily\bfseries\small,
  identifierstyle=\small,
%  commentline=\%,
  keywords={assumes,automaton,axioms,backward,bounds,by,case,choose,components,const,d,det,discrete,do,eff,else,elseif,ensuring,enumeration,evolve,fi,fire,follow,for,forward,from,hidden,if,in,%
    input,initially,internal,invariant,let, local,od,of,output,pre,schedule,signature,so,%
    simulation,states,variables, tasks, stop,tasks,that,then,to,trajdef,trajectory,trajectories,transitions,tuple,type,union,urgent,uses,when,where,while,yield},
  literate=
        % LaTeX math symbols
        {\\in}{{$\in$}}1
        {\\preceq}{{$\preceq$}}1
        {\\subset}{{$\subset$}}1
        {\\subseteq}{{$\subseteq$}}1
        {\\supset}{{$\supset$}}1
        {\\supseteq}{{$\supseteq$}}1
        {\\rho}{{$\rho$}}1
        {\\infty}{{$\infty$}}1
        % LSL symbols (one-character)
        {<}{{$<$}}1
        {>}{{$>$}}1
        {=}{{$=$}}1
        {~}{{$\neg$}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall$}}1 {\\E}{{$\exists$}}1
        {\\/}{{$\vee$}}1 {/\\}{{$\wedge$}}1
        {=>}{{$\Rightarrow$}}1
        {->}{{$\rightarrow$}}1
        {<=}{{$\leq$}}1 {>=}{{$\geq$}}1 {~=}{{$\neq$}}1
        {\\U}{{$\cup$}}1 {\\I}{{$\cap$}}1
        {|-}{{$\vdash$}}1 {-|}{{$\dashv$}}1
        {<<}{{$\ll$}}2 {>>}{{$\gg$}}2
        {||}{{$\|$}}1
%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
        % LSL symbols (three or more characters)
        {<=>}{{$\Leftrightarrow$}}2
        {<->}{{$\leftrightarrow$}}2
        {(+)}{{$\oplus$}}1
        {(-)}{{$\ominus$}}1
}

\lstdefinelanguage{bigIOALang}{%
  basicstyle=\ttfamily,
  keywordstyle=\rmfamily\bfseries,
  identifierstyle=,
%  commentline=\%,
  keywords={assumes,automaton,axioms,backward,by,case,choose,components,const,%
    d,det,discrete,do,eff,else,elseif,ensuring,enumeration,evolve,fi,for,forward,from,hidden,if,in%
    input,initially,internal,invariant,local,od,of,output,pre,schedule,signature,so,%
    tasks, simulation,states,stop,tasks,that,then,to,trajdef,trajectories,transitions,tuple,type,union,urgent,uses,when,where,yield},
  literate=
        % LaTeX math symbols
        {\\in}{{$\in$}}1
        {\\preceq}{{$\preceq$}}1
        {\\subset}{{$\subset$}}1
        {\\subseteq}{{$\subseteq$}}1
        {\\supset}{{$\supset$}}1
        {\\supseteq}{{$\supseteq$}}1
        % LSL symbols (one-character)
        {<}{{$<$}}1
        {>}{{$>$}}1
        {=}{{$=$}}1
        {~}{{$\neg$}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall$}}1 {\\E}{{$\exists$}}1
        {\\/}{{$\vee$}}1 {/\\}{{$\wedge$}}1
        {=>}{{$\Rightarrow$}}1
        {->}{{$\rightarrow$}}1
        {<=}{{$\leq$}}1 {>=}{{$\geq$}}1 {~=}{{$\neq$}}1
        {\\U}{{$\cup$}}1 {\\I}{{$\cap$}}1
        {|-}{{$\vdash$}}1 {-|}{{$\dashv$}}1
        {<<}{{$\ll$}}2 {>>}{{$\gg$}}2
        {||}{{$\|$}}1
%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
        % LSL symbols (three or more characters)
        {<=>}{{$\Leftrightarrow$}}2
        {<->}{{$\leftrightarrow$}}2
        {(+)}{{$\oplus$}}1
        {(-)}{{$\ominus$}}1
}


\lstnewenvironment{BigIOA}%
  {\lstset{language=bigIOALang,basicstyle=\ttfamily}
   \csname lst@SetFirstLabel\endcsname}
  {\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}

\lstnewenvironment{SmallIOA}%
  {\lstset{language=ioaLang,basicstyle=\ttfamily\scriptsize}
   \csname lst@SetFirstLabel\endcsname}
  %{\csname lst@SaveFirstLabel\endcsname\vspace{-4pt}\noindent}
  {\csname lst@SaveFirstLabel\endcsname\noindent}


\newcommand{\true}{\relax\ifmmode \mathit true \else \em true \/\fi}
\newcommand{\false}{\relax\ifmmode \mathit false \else \em false \/\fi}



\newcommand{\Real}{{\operatorname{\texttt{Real}}}}
\newcommand{\Bool}{{\operatorname{\texttt{Bool}}}}
\newcommand{\Char}{{\operatorname{\texttt{Char}}}}
\newcommand{\ioaInt}{{\operatorname{\texttt{Int}}}}
\newcommand{\ioaNat}{{\operatorname{\texttt{Nat}}}}
\newcommand{\ioaAugR}{{\operatorname{\texttt{AugmentedReal}}}}
\newcommand{\ioaString}{{\operatorname{\texttt{String}}}}
\newcommand{\Discrete}{{\operatorname{\texttt{Discrete}}}}
%\newcommand{\Bool}{{\operatorname{\texttt{Bool}}}}

%\newcommand{\lnot}{\neg}
%\newcommand{\land}{\wedge}
%\newcommand{\lor}{\vee}
\newcommand{\limplies}{\Rightarrow}
\newcommand{\liff}{\Leftrightarrow}

\newlength{\bracklen}
\newcommand{\sem}[1]{\settowidth{\bracklen}{[}
     [\hspace{-0.5\bracklen}[#1]\hspace{-0.5\bracklen}]}

\newcommand{\defaultArraystretch}{1.4}
\renewcommand{\arraystretch}{\defaultArraystretch}

\newcommand{\gS}{\mathcal{S}}
\newcommand{\gV}{\mathcal{V}}
\newcommand{\freevars}{\mathcal{FV}}

\newcommand{\gVspec}{\mathcal{V}_\mathit{spec}}
\newcommand{\gVa}{\mathcal{V}_\mathit{A}}
\newcommand{\gVsig}{\mathcal{V}_\mathit{sigs}}
\newcommand{\gVso}{\mathcal{V}_\mathit{sorts}}
\newcommand{\gVop}{\mathcal{V}_\mathit{ops}}
\newcommand{\sort}{\mathit{sort}}
\newcommand{\sig}{\mathit{sig}}
\newcommand{\id}{\mathit{id}}
\newcommand{\sigsep}{\lsl`->`}

%\newcommand{\T}{\mathit{true}}
%\newcommand{\F}{\mathit{false}}

\newcommand{\super}[2]{\ensuremath{\mathit{#1}^\mathit{#2}}}
\newcommand{\tri}[3]{\ensuremath{\mathit{#1}^\mathit{#2}_\mathit{#3}}}
\newcommand{\Assumptions}{\ensuremath{\mathit{Assumptions}}}
\newcommand{\actPred}[3][\pi]{\tri{P}{#2,#1}{#3}}
\newcommand{\actualTypes}[1]{\super{actualTypes}{#1}}
\newcommand{\actuals}[1]{\super{actuals}{#1}}
\newcommand{\autActVars}[2][\pi]{\vars{#2}{},\vars{#2,#1}{}}
\newcommand{\bracket}[2]{\mathit{#1}[\mathit{#2}]}
\newcommand{\compVars}[1]{\super{compVars}{#1}}
\newcommand{\context}{\mathit{context}}
\newcommand{\ensuring}[2]{\tri{ensuring}{#1}{#2}}
\newcommand{\initPred}[1]{\tri{P}{#1}{init}}
\newcommand{\initVals}[1]{\super{initVals}{#1}}
\newcommand{\initially}[2]{\tri{initially}{#1}{#2}}
\newcommand{\invPred}[2]{\tri{Inv}{#1}{#2}}
\newcommand{\knownVars}[1]{\super{knownVars}{#1}}
\newcommand{\localPostVars}[2]{\tri{localPostVars}{#1}{#2}}
\newcommand{\localVars}[2]{\tri{localVars}{#1}{#2}}
\newcommand{\locals}[1]{\bracket{Locals}{#1}}
\newcommand{\nam}[1]{\rho^{\mathit{#1}}}
\newcommand{\otherActPred}[3][\pi]{\otherTri{P}{#2,#1}{#3}}
\newcommand{\otherParams}[2]{\otherTri{params}{#1}{#2}}
\newcommand{\otherSub}[2]{\otherTri{\sigma}{#1}{#2}}
\newcommand{\otherTri}[3]{\tri{\smash{#1'}}{#2}{#3}}
\newcommand{\otherVars}[2]{\otherTri{vars}{#1}{#2}}
\newcommand{\params}[2]{\tri{params}{#1}{#2}}
\newcommand{\postVars}[1]{\super{postVars}{#1}}
\newcommand{\pre}[2]{\tri{Pre}{#1}{#2}}
\newcommand{\prog}[2]{\tri{Prog}{#1}{#2}}
\newcommand{\prov}[2]{\tri{Prov}{#1}{#2}}
\newcommand{\stateSorts}[1]{\super{stateSorts}{#1}}
\newcommand{\stateVars}[1]{\super{stateVars}{#1}}
\newcommand{\states}[1]{\bracket{States}{#1}}
%\newcommand{\sub}[2]{\tri{\sigma}{#1}{#2}}
\newcommand{\sugActPred}[3][\pi]{\tri{P}{#2,#1}{#3,desug}}
\newcommand{\sugLocalVars}[2]{\ifthenelse{\equal{}{#2}}%
                             {\tri{localVars}{#1}{desug}}%
                             {\tri{localVars}{#1}{#2,desug}}}
\newcommand{\sugVars}[2]{\ifthenelse{\equal{}{#2}}%
                        {\tri{vars}{#1}{desug}}%
                        {\tri{vars}{#1}{#2,desug}}}
\newcommand{\cVars}[1]{\super{cVars}{#1}}

\newcommand{\vmap}{\dot{\varrho}}
\newcommand{\map}[2]{\tri{\vmap}{#1}{#2}}

\newcommand{\types}[1]{\super{types}{#1}}
\newcommand{\vars}[2]{\tri{vars}{#1}{#2}}

\newcommand{\subActPred}[3][\pi]{\sub{#2,#1}{#3}(\tri{P}{#2,#1}{#3,desug})}
\newcommand{\subLocalVars}[2]{\sub{#1}{#2}(\tri{localVars}{#1}{#2,desug})}

\newcommand{\dA}{\hat{A}}
\newcommand{\renameAction}[1]{\ensuremath{\rho_{#1}(\vars{\dA{#1},\pi}{})}}
\newcommand{\renameComponent}[1]{\ensuremath{\rho_{#1}\dA_{#1}}}

\newenvironment{Syntax}{\[\begin{subSyntax}}{\end{subSyntax}\]\vspace{-.3in}}
\newenvironment{subSyntax}{\begin{array}{l}}{\end{array}}
%\newcommand{\w}[1]{\mbox{\hspace*{#1em}}}



%TIOA macros
% Script math symbol name
\newcommand{\ms}[1]{\ifmmode%
\mathord{\mathcode`-="702D\it #1\mathcode`\-="2200}\else%
$\mathord{\mathcode`-="702D\it #1\mathcode`\-="2200}$\fi}

%\newcommand{\domain}[1]{{\it dom}(#1)} % domain

% KEYWORDS
\newcommand{\kw}[1]{{\bf #1}}
\newcommand{\tcon}[1]{{\tt #1}}
\newcommand{\syn}[1]{{\tt #1}}
\newcommand{\pvskw}[1]{{\sc #1}}
\newcommand{\pvsid}[1]{{\operatorname{\mathit{#1}}}}


% TIMED AUTOMATA
\def\A{{\cal A}} % TA
\def\B{{\cal B}} % TA
\def\D{{\cal D}} % set of discrete steps
\def\T{{\cal T}} % set of trajectories

% VALUATIONS
\newcommand{\vv}{{\bf v}}
\newcommand{\vw}{{\bf w}}
\newcommand{\vx}{{\bf x}}
\newcommand{\vy}{{\bf y}}
\newcommand{\va}{{\bf a}}
\newcommand{\vb}{{\bf b}}
\newcommand{\vc}{{\bf c}}
\newcommand{\vq}{{\bf q}}
\newcommand{\vs}{{\bf s}}
\newcommand{\vm}{{\bf m}}
\newcommand{\vu}{{\bf u}}

% Transitions and trajectory operations
\newcommand{\arrow}[1]{\mathrel{\stackrel{#1}{\rightarrow}}}
\newcommand{\sarrow}[2]{\mathrel{\stackrel{#1}{\rightarrow_{#2}}}}
\newcommand{\concat}{\mathbin{^{\frown}}} % concatenation
\newcommand{\paste}{\mathrel{\diamond}}

% AUTOMATA
%\def\A{{\cal A}}
%\def\B{{\cal B}}
%\def\T{{\cal T}} % set of trajectories

\def\CC{{\mathscr C}} % concatenation closure

% PVS STUFF

\lstdefinelanguage{pvs}{
  basicstyle=\tt \figuresize,
  keywordstyle=\sc \figuresize,
  identifierstyle=\it \figuresize,
  emphstyle=\tt \figuresize,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={and,
  	 begin,
  	 cases, const,
  	 do,
  	 external, else, exists, end, endcases, endif,
  	 fi,for, forall, from,
  	 hidden,
  	 in, if, importing,
     let, lambda, lemma,
     measure,
     not,
     or, of,
     return, recursive,
     stop,
     theory, that,then, type, types, type+, to, theorem,
     var,
     with,while},
  emph={nat, setof, sequence, eq, tuple, map, array, enumeration, bool, real, exp, nnreal, posreal},
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\mapsto}{{$\rightarrow\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {->}{{$\rightarrow\ $}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3
      }



\lstdefinelanguage{BigPVS}{
  basicstyle=\tt,
  keywordstyle=\sc,
  identifierstyle=\it,
  emphstyle=\tt ,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={and,
  	 begin,
  	 cases, const,
  	 do, datatype,
  	 external, else, exists, end, endif, endcases,
  	 fi,for, forall, from,
  	 hidden,
  	 in, if, importing,
     let, lambda, lemma,
     measure,
     not,
     or, of,
     return, recursive,
     stop,
     theory, that,then, type, types, type+, to, theorem,
     var,
     with,while},
  emph={nat, setof, sequence, eq, tuple, map, array, first, rest, add, enumeration, bool, real, posreal, nnreal},
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\mapsto}{{$\rightarrow\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {->}{{$\rightarrow\ $}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3
      }

\lstdefinelanguage{pvsNums}[]{pvs}
{
  numbers=left,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\lstdefinelanguage{pvsNumsRight}[]{pvs}
{
  numbers=right,
  numberstyle=\tiny,
  stepnumber=2,
  numbersep=4pt
%  firstnumber=1
}

\newcommand{\pvs}{\lstinline[language=PVS]}

\lstnewenvironment{BigPVS}%
  {\lstset{language=BigPVS}}
  {}

\lstnewenvironment{PVSNums}%
  {
  \if@firstcolumn
    \lstset{language=pvs, numbers=left, firstnumber=auto}
  \else
    \lstset{language=pvs, numbers=right, firstnumber=auto}
  \fi
  }
  {}

\lstnewenvironment{PVSNumsRight}%
  {
    \lstset{language=pvs, numbers=right, firstnumber=auto}
  }
  {}


\newcommand{\figpvs}[5]{
  \begin{figure}[#1]
      \hrule \F
      {\figuresize \bf #2}
      \lstinputlisting[language=pvs]{#5}
      \F \hrule \F
      \caption{#3}
      \label{fig: #4}
  \end{figure}
}

\newcommand{\linefigpvs}[9]{

}

\newcommand{\twofigpvs}[8]{
  \begin{figure}[#1]
    \hrule \F
    {\figuresize \bf #2} \\
    \two{#5}{#6}
    {
      \lstinputlisting[language=pvsLang]{#7}
    }
    {
      \lstinputlisting[language=pvsLang]{#8}
    }
    \F \hrule \F
    \caption{#3}
    \label{fig: #4}
  \end{figure}
}


\lstdefinelanguage{pvsproof}{
  basicstyle=\tt \figuresize,
  mathescape=true,
  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
  basewidth=0.05em,
}


\lstdefinelanguage{pseudo}{
  basicstyle=\figuresize,
  keywordstyle=\bf \figuresize,
  identifierstyle=\it \figuresize,
  emphstyle=\tt \figuresize,
  mathescape=true,
  tabsize=20,
%  tabsize=4,
  sensitive=false,
  columns=fullflexible,
  keepspaces=false,
  flexiblecolumns=true,
%  basewidth=0.5em,
  basewidth=0.05em,
  moredelim=[il][\rm]{//},
  moredelim=[is][\sf \figuresize]{!}{!},
  moredelim=[is][\bf \figuresize]{*}{*},
  keywords={automaton,and,
  	 choose,const,continue, components,
  	 discrete, do,
  	 eff, external,else, elseif, evolve, end,
  	 fi,for, forward, from,
  	 hidden,
  	 in,input,internal,if,invariant, initially, imports,
     let,
     or, output, operators, od, of,
     pre,
     return, round,
     such,satisfies, stop, signature, simulation,
     trajectories,trajdef, transitions, that,then, type, types, to, tasks,
     upon,
     variables, vocabulary,
     wait, when,where, with,while},
  emph={set, seq, tuple, map, array, enumeration},
   literate=
        {(}{{$($}}1
        {)}{{$)$}}1
        % LaTeX math symbols
        {\\in}{{$\in\ $}}1
        {\\preceq}{{$\preceq\ $}}1
        {\\subset}{{$\subset\ $}}1
        {\\subseteq}{{$\subseteq\ $}}1
        {\\supset}{{$\supset\ $}}1
        {\\supseteq}{{$\supseteq\ $}}1
        {\\forall}{{$\forall$}}1
        {\\le}{{$\le\ $}}1
        {\\ge}{{$\ge\ $}}1
        {\\gets}{{$\gets\ $}}1
        {\\cup}{{$\cup\ $}}1
        {\\cap}{{$\cap\ $}}1
        {\\langle}{{$\langle$}}1
        {\\rangle}{{$\rangle$}}1
        {\\exists}{{$\exists\ $}}1
        {\\bot}{{$\bot$}}1
        {\\rip}{{$\rip$}}1
        {\\emptyset}{{$\emptyset$}}1
        {\\notin}{{$\notin\ $}}1
        {\\not\\exists}{{$\not\exists\ $}}1
        {\\ne}{{$\ne\ $}}1
        {\\to}{{$\to\ $}}1
        {\\implies}{{$\implies\ $}}1
        % LSL symbols (one-character)
        {<}{{$<\ $}}1
        {>}{{$>\ $}}1
        {=}{{$=\ $}}1
        {~}{{$\neg\ $}}1
        {|}{{$\mid$}}1
        {'}{{$^\prime$}}1
        % LSL symbols (two characters)
        {\\A}{{$\forall\ $}}1
        {\\E}{{$\exists\ $}}1
        {\\/}{{$\vee\,$}}1
        {\\vee}{{$\vee\,$}}1
        {/\\}{{$\wedge\,$}}1
        {\\wedge}{{$\wedge\,$}}1
        {=>}{{$\Rightarrow\ $}}1
        {->}{{$\rightarrow\ $}}1
        {<=}{{$\Leftarrow\ $}}1
        {<-}{{$\leftarrow\ $}}1
%        {<=}{{$\leq$}}1
%        {>=}{{$\geq$}}1
        {~=}{{$\neq\ $}}1
        {\\U}{{$\cup\ $}}1
        {\\I}{{$\cap\ $}}1
        {|-}{{$\vdash\ $}}1
        {-|}{{$\dashv\ $}}1
        {<<}{{$\ll\ $}}2
        {>>}{{$\gg\ $}}2
        {||}{{$\|$}}1
%%       {\[\]}{{\[\,\]}}2 {\{\}}{{\{\,\}}}2
%%        {[}{{$\langle$}}1
%%        {]}{{$\rangle$}}1
        {[}{{$[$}}1
        {]}{{$\,]$}}1
        {[[}{{$\langle$}}1
        {]]]}{{$]\rangle$}}1
        {]]}{{$\rangle$}}1
        {<=>}{{$\Leftrightarrow\ $}}2
        {<->}{{$\leftrightarrow\ $}}2
        {(+)}{{$\oplus\ $}}1
        {(-)}{{$\ominus\ $}}1
        {_i}{{$_{i}$}}1
        {_j}{{$_{j}$}}1
        {_{i,j}}{{$_{i,j}$}}3
        {_{j,i}}{{$_{j,i}$}}3
        {_0}{{$_0$}}1
        {_1}{{$_1$}}1
        {_2}{{$_2$}}1
        {_n}{{$_n$}}1
        {_p}{{$_p$}}1
        {_k}{{$_n$}}1
        {-}{{$\ms{-}$}}1
        {@}{{}}0
        {\\delta}{{$\delta$}}1
        {\\R}{{$\R$}}1
        {\\Rplus}{{$\Rplus$}}1
        {\\N}{{$\N$}}1
        {\\times}{{$\times\ $}}1
        {\\tau}{{$\tau$}}1
        {\\alpha}{{$\alpha$}}1
        {\\beta}{{$\beta$}}1
        {\\gamma}{{$\gamma$}}1
        {\\ell}{{$\ell\ $}}1
        {--}{{$-\ $}}1
        {\\TT}{{\hspace{1.5em}}}3
      }

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\pair}[1]{\left\langle#1\right\rangle}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\norm}[1]{\left\lvert\left\lvert#1\right\rvert\right\rvert}
\newcommand{\argmin}[2]{\underset{#2}{\operatorname{argmin}} #1}
\newcommand{\argmax}[2]{\underset{#2}{\operatorname{argmax}} #1}
\newcommand{\maxel}[2]{\underset{#2}{\operatorname{max}} #1}
\newcommand{\minel}[2]{\underset{#2}{\operatorname{min}} #1}
\newcommand{\supel}[2]{\underset{#2}{\operatorname{sup}} #1}
\newcommand{\infel}[2]{\underset{#2}{\operatorname{inf}} #1}
\newcommand{\sgn}[1]{\operatorname{sgn} \left( #1 \right)}
\newcommand{\lima}[2]{\underset{#2}{\operatorname{lim}} #1}
\newcommand{\ds}[1]{\left\llbracket#1\right\rrbracket}	%denotation of states

\newcommand{\deq}{\mathrel{\stackrel{\scriptscriptstyle\Delta}{=}}}

%\renewenvironment{proof}[1][Proof]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\qed\end{trivlist}}
%\newenvironment{proof}{\trivlist\item[]\emph{Proof}:}{\unskip\nobreak\hskip 1em plus 1fil\nobreak\qed\parfillskip=0pt\endtrivlist}
\newenvironment{proofof}[1]{\trivlist\item[]\emph{Proof of #1}:}{\unskip\nobreak\hskip 1em plus 1fil\nobreak\qed\parfillskip=0pt\endtrivlist}

\def\Rq{\sim}
%\def\Aq{\A_q}

\def\nuh{\hat{\nu}}
\def\Vi{\vec{V}_I}
\def\Vt{\vec{V}_T}
%\def\Vv{\vec{\Delta} V }

\def\dnumin{\dot{\nu}_{2min}}
\def\dnumax{\dot{\nu}_{2max}}


%define reach sets used in iccps 2012 and in conjunction avoidance


\newcommand{\reacht}[1]{\relax\ifmmode {\sf Reach}_{#1}(t) \else ${\sf Reach}_{#1}(t)$\fi}

\newcommand{\reachi}[2]{\relax\ifmmode {\sf Reach}_{#1}(#2) \else ${\sf Reach}_{#1}(#2)$\fi}

\newcommand{\breach}[2]{\relax\ifmmode {\sf Reach}^{#2}_{#1} \else ${\sf Reach}^{#2}_{#1}$\fi}

\newcommand{\breachi}[3]{\relax\ifmmode {\sf Reach}^{#2}_{#1}(#3) \else ${\sf Reach}^{#2}_{#1}(#3)$\fi}

\newcommand{\breacht}[2]{\relax\ifmmode {\sf Reach}^{#2}_{#1}(t) \else ${\sf Reach}^{#2}_{#1}(t)$\fi}


%indentation for algorithmic
\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

%reach set composisiton
\def\rcomp{C}

% leaf node of the verify algorithm call tree
\def\leaf{\sigma}

%definition of queue
\def\queue{\Omega}

%definition of time bound for bounded time reach sets
\def\tbound{T}

% definition for external variables
\def\evarset{Y}
\def\evar{y}

% time partition variable and corresponding index set
\def\timepart{\Gamma}
\def\timeset{\I}


% abstraction for automata composition
% \newcommand{\comp}[1]{ {#1}^{\#} }
\newcommand{\comp}[1]{ {#1}' }

% error term for convergence of abstraction analysis
\def\error{e}

% define a vector form to be used for variables
\newcommand{\varvec}[1]{ \mathbf{#1} }




\def\DeltaV{\overrightarrow{\Delta V}}


\def\capright{\textbf{(Right)}\xspace}
\def\capleft{\textbf{(Left)}\xspace}

\def\interior{\circ}



